An Early-Time Optical and Ultraviolet Excess in the type-Ic SN 2020oi

We present photometric and spectroscopic observations of Supernova 2020oi (SN 2020oi), a nearby ($\sim$17 Mpc) type-Ic supernova (SN Ic) within the grand-design spiral M100. We undertake a comprehensive analysis to characterize the evolution of SN 2020oi and constrain its progenitor system. We detect flux in excess of the fireball rise model $\delta t \approx 2.5$ days from the date of explosion in multi-band optical and UV photometry from the Las Cumbres Observatory and the Neil Gehrels Swift Observatory, respectively. The derived SN bolometric luminosity is consistent with an explosion with $M_{\rm ej} = 0.81 \pm 0.03 M_{\odot}$, $E_{k}= 0.79 \pm 0.09 \times 10^{51} \rm{erg} \rm{s}^{-1}$, and $M_{\rm Ni56} = 0.08 \pm 0.02 M_{\odot}$. Inspection of the event's decline reveals the highest $\Delta m_{15,\rm{bol}}$ reported for a stripped-envelope event to date. Modeling of optical spectra near event peak indicates a partially mixed ejecta comparable in composition to the ejecta observed in SN 1994I, while the earliest spectrum shows signatures of a possible interaction with material of a distinct composition surrounding the SN progenitor. Further, Hubble Space Telescope (HST) pre-explosion imaging reveals a stellar cluster coincident with the event. From the cluster photometry, we derive the mass and age of the SN progenitor using stellar evolution models implemented in the BPASS library. Our results indicate that SN 2020oi occurred in a binary system from a progenitor of mass $M_{\rm ZAMS} \approx 9.5 \pm 1.0 M_{\odot}$, corresponding to an age of $27 \pm 7$ Myr. SN 2020oi is the dimmest SN Ic event to date for which an early-time flux excess has been observed, and the first in which an early excess is unlikely to be associated with shock-cooling.

==> phottable_bak_old.tex <==
\begin{table}[]
\parbox{.45\linewidth}{

\centering \caption {Optical and UV Photometry of SN~2020oi} \label{tbl:optical_phot} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58856.46 & +2.26   & $UVW2$ & $>$18.3   & --     & $Swift$   \\
58856.79 & +2.59   & $UVW2$ & $>$18.028 & --     & $Swift$   \\
58857.45 & +3.25   & $UVW2$ & $>$18.587 & --     & $Swift$   \\
58858.85 & +4.65   & $UVW2$ & $>$18.212 & --     & $Swift$   \\
58859.49 & +5.29   & $UVW2$ & $>$18.465 & --     & $Swift$   \\
58860.38 & +6.18   & $UVW2$ & $>$18.375 & --     & $Swift$   \\
58861.25 & +7.05   & $UVW2$ & $>$18.201 & --     & $Swift$   \\
58877.19 & +22.99  & $UVW2$ & $>$18.476 & --     & $Swift$   \\
58887.68 & +33.48  & $UVW2$ & $>$18.451 & --     & $Swift$   \\
58898.57 & +44.37  & $UVW2$ & $>$18.539 & --     & $Swift$   \\
58907.25 & +53.05  & $UVW2$ & $>$18.425 & --     & $Swift$   \\
58856.46 & +2.26   & $UVM2$ & $>$18.109 & --     & $Swift$   \\
58857.46 & +3.26   & $UVM2$ & $>$18.243 & --     & $Swift$   \\
58858.86 & +4.66   & $UVM2$ & $>$18.169 & --     & $Swift$   \\
58860.38 & +6.18   & $UVM2$ & $>$18.356 & --     & $Swift$   \\
58861.25 & +7.05   & $UVM2$ & $>$18.235 & --     & $Swift$   \\
58877.19 & +22.99  & $UVM2$ & $>$18.402 & --     & $Swift$   \\
58887.68 & +33.48  & $UVM2$ & $>$18.376 & --     & $Swift$   \\
58898.57 & +44.37  & $UVM2$ & $>$18.546 & --     & $Swift$   \\
58907.25 & +53.05  & $UVM2$ & $>$18.323 & --     & $Swift$   \\
58856.45 & +2.25   & $UVW1$ & 18.919               & 0.707  & $Swift$   \\
58856.79 & +2.59   & $UVW1$ & 18.509               & 0.615  & $Swift$   \\
58857.45 & +3.25   & $UVW1$ & $>$18.332 & --     & $Swift$   \\
58858.84 & +4.64   & $UVW1$ & 18.478               & 0.531  & $Swift$   \\
58859.48 & +5.28   & $UVW1$ & 18.542               & 0.68   & $Swift$   \\
58859.81 & +5.61   & $UVW1$ & 18.378               & 0.627  & $Swift$   \\
58859.97 & +5.77   & $UVW1$ & 18.172               & 0.453  & $Swift$   \\
58860.38 & +6.18   & $UVW1$ & 18.637               & 0.563  & $Swift$   \\
58861.24 & +7.04   & $UVW1$ & 17.48                & 0.249  & $Swift$   \\
58877.19 & +22.99  & $UVW1$ & 19.257               & 0.93   & $Swift$   \\
58887.68 & +33.48  & $UVW1$ & $>$18.397 & --     & $Swift$   \\
58898.57 & +44.37  & $UVW1$ & $>$18.333 & --     & $Swift$   \\
58907.25 & +53.05  & $UVW1$ & $>$18.359 & --     & $Swift$   \\
58857.3  & +3.1    & $u$    & 16.043               & 0.09   & LCO       \\
58857.3  & +3.1    & $u$    & 16.043               & 0.09   & LCO       \\
58860.42 & +6.22   & $u$    & -11.156              & 1.086  & LCO       \\
58861.05 & +6.85   & $u$    & 15.361               & 1.086  & LCO       \\
58861.05 & +6.85   & $u$    & 14.738               & 0.031  & LCO       \\
58872.35 & +18.15  & $u$    & 16.748               & 0.0    & Swope     \\
58876.33 & +22.13  & $u$    & 14.659               & 1.086  & LCO       \\
58876.37 & +22.17  & $u$    & 18.101               & 0.031  & Swope     \\
58882.32 & +28.12  & $u$    & 18.626               & 0.041  & Swope     \\
58884.37 & +30.17  & $u$    & 16.356               & 1.086  & LCO       \\
58885.36 & +31.16  & $u$    & 18.754               & 0.069  & Swope     \\
58893.29 & +39.09  & $u$    & 17.173               & 0.0    & Swope     \\
58895.29 & +41.09  & $u$    & 16.077               & 1.086  & LCO       \\
58895.29 & +41.09  & $u$    & 19.182               & 0.085  & Swope     \\
58896.29 & +42.09  & $u$    & 19.011               & 0.11   & Swope     \\
58897.32 & +43.12  & $u$    & 18.058               & 0.022  & Swope     \\
58902.24 & +48.04  & $u$    & 15.442               & 1.086  & LCO       \\
58903.28 & +49.08  & $u$    & 19.184               & 0.095  & Swope     \\
58904.33 & +50.13  & $u$    & 19.24                & 0.066  & Swope     \\ \hline
\end{tabular}
}
\hfill
\parbox{.45\linewidth}
{
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58905.29 & +51.09  & $u$    & 19.288               & 0.068  & Swope     \\
58906.1  & +51.9   & $u$    & 16.261               & 1.086  & LCO       \\
58906.28 & +52.08  & $u$    & 19.406               & 0.077  & Swope     \\
58907.37 & +53.17  & $u$    & 19.017               & 0.074  & Swope     \\
58908.31 & +54.11  & $u$    & 19.282               & 0.1    & Swope     \\
58909.36 & +55.16  & $u$    & 19.231               & 0.066  & Swope     \\
58910.16 & +55.96  & $u$    & 16.405               & 1.086  & LCO       \\
58910.25 & +56.05  & $u$    & 19.224               & 0.092  & Swope     \\
58911.2  & +57.0   & $u$    & 19.189               & 0.089  & Swope     \\
58912.27 & +58.07  & $u$    & 19.433               & 0.111  & Swope     \\
58919.14 & +64.94  & $u$    & 16.446               & 1.086  & LCO       \\
58921.25 & +67.05  & $u$    & 18.08                & 0.067  & Swope     \\
58923.14 & +68.94  & $u$    & 16.64                & 1.086  & LCO       \\
58929.5  & +75.3   & $u$    & 17.573               & 0.092  & LCO       \\
58929.5  & +75.3   & $u$    & 16.924               & 1.086  & LCO       \\
58935.62 & +81.42  & $u$    & 15.52                & 0.362  & LCO       \\
58935.62 & +81.42  & $u$    & 15.52                & 1.086  & LCO       \\
58935.64 & +81.44  & $u$    & 15.634               & 0.362  & LCO       \\
58935.64 & +81.44  & $u$    & 15.634               & 1.086  & LCO       \\
58943.46 & +89.26  & $u$    & 15.305               & 0.362  & LCO       \\
58943.46 & +89.26  & $u$    & 15.305               & 1.086  & LCO       \\
58952.44 & +98.24  & $u$    & 16.709               & 1.086  & LCO       \\
58966.35 & +112.15 & $u$    & 16.961               & 1.086  & LCO       \\
58974.11 & +119.91 & $u$    & 16.272               & 1.086  & LCO       \\
58980.76 & +126.56 & $u$    & 17.511               & 1.086  & LCO       \\
58988.31 & +134.11 & $u$    & 16.678               & 1.086  & LCO       \\
58996.5  & +142.3  & $u$    & 17.33                & 1.086  & LCO       \\
59002.74 & +148.54 & $u$    & 18.82                & 1.086  & LCO       \\
59007.7  & +153.5  & $u$    & 19.422               & 1.086  & LCO       \\
59014.79 & +160.59 & $u$    & 19.652               & 1.086  & LCO       \\
59026.34 & +172.14 & $u$    & 18.543               & 1.086  & LCO       \\
59032.34 & +178.14 & $u$    & 19.931               & 1.086  & LCO       \\
59202.09 & +347.89 & $u$    & 18.463               & 1.086  & LCO       \\
59208.07 & +353.87 & $u$    & 18.475               & 1.086  & LCO       \\
59213.45 & +359.25 & $u$    & 17.213               & 1.086  & LCO       \\
59214.05 & +359.85 & $u$    & 17.37                & 1.086  & LCO       \\
59220.37 & +366.17 & $u$    & 18.04                & 1.086  & LCO       \\
59226.1  & +371.9  & $u$    & 18.408               & 1.086  & LCO       \\
59227.71 & +373.51 & $u$    & 18.378               & 1.086  & LCO       \\
59232.37 & +378.17 & $u$    & 17.759               & 1.086  & LCO       \\
59236.06 & +381.86 & $u$    & 17.924               & 1.086  & LCO       \\
59245.42 & +391.22 & $u$    & 18.394               & 1.086  & LCO       \\
59252.05 & +397.85 & $u$    & 18.802               & 1.086  & LCO       \\
59257.33 & +403.13 & $u$    & 18.371               & 1.086  & LCO       \\
59262.22 & +408.02 & $u$    & 18.188               & 1.086  & LCO       \\
59267.12 & +412.92 & $u$    & 17.542               & 1.086  & LCO       \\
58856.45 & +2.25   & $U$    & 16.672               & 0.182  & $Swift$   \\
58856.79 & +2.59   & $U$    & 16.677               & 0.198  & $Swift$   \\
58857.45 & +3.25   & $U$    & 17.069               & 0.229  & $Swift$   \\
58858.85 & +4.65   & $U$    & 16.578               & 0.173  & $Swift$   \\
58859.49 & +5.29   & $U$    & 16.302               & 0.175  & $Swift$   \\
58860.38 & +6.18   & $U$    & 15.883               & 0.124  & $Swift$   \\ \hline
\end{tabular}
}
\end{table}



\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58861.25 & +7.05   & $U$    & 15.466               & 0.109  & $Swift$   \\
58877.19 & +22.99  & $U$    & $>$17.64  & --     & $Swift$   \\
58887.68 & +33.48  & $U$    & $>$17.513 & --     & $Swift$   \\
58887.69 & +33.49  & $U$    & $>$17.762 & --     & $Swift$   \\
58898.56 & +44.36  & $U$    & $>$17.631 & --     & $Swift$   \\
58898.57 & +44.37  & $U$    & $>$17.813 & --     & $Swift$   \\
58907.25 & +53.05  & $U$    & $>$17.626 & --     & $Swift$   \\
58907.26 & +53.06  & $U$    & $>$17.789 & --     & $Swift$   \\
58856.45 & +2.25   & $B$    & 16.463               & 0.203  & $Swift$   \\
58856.79 & +2.59   & $B$    & 16.589               & 0.228  & $Swift$   \\
58857.45 & +3.25   & $B$    & 16.542               & 0.213  & $Swift$   \\
58858.85 & +4.65   & $B$    & 15.823               & 0.143  & $Swift$   \\
58859.49 & +5.29   & $B$    & 15.687               & 0.151  & $Swift$   \\
58860.38 & +6.18   & $B$    & 15.298               & 0.113  & $Swift$   \\
58861.25 & +7.05   & $B$    & 14.874               & 0.099  & $Swift$   \\
58869.35 & +15.15  & $B$    & 15.112               & 0.012  & Swope     \\
58869.35 & +15.15  & $B$    & 15.261               & 0.005  & Swope     \\
58870.32 & +16.12  & $B$    & 15.415               & 0.007  & Swope     \\
58871.36 & +17.16  & $B$    & 15.667               & 0.006  & Swope     \\
58872.36 & +18.16  & $B$    & 15.831               & 0.004  & Swope     \\
58873.09 & +18.89  & $B$    & 18.624               & 1.086  & LCO       \\
58875.38 & +21.18  & $B$    & 16.357               & 0.014  & Swope     \\
58876.37 & +22.17  & $B$    & 16.47                & 0.005  & Swope     \\
58878.06 & +23.86  & $B$    & 16.787               & 1.086  & LCO       \\
58879.07 & +24.87  & $B$    & 16.469               & 1.086  & LCO       \\
58880.44 & +26.24  & $B$    & 18.829               & 1.086  & Nickel    \\
58882.33 & +28.13  & $B$    & 17.035               & 0.006  & Swope     \\
58883.01 & +28.81  & $B$    & 18.078               & 1.086  & LCO       \\
58883.38 & +29.18  & $B$    & 17.086               & 0.008  & Swope     \\
58884.38 & +30.18  & $B$    & 17.074               & 0.008  & Swope     \\
58885.37 & +31.17  & $B$    & 17.154               & 0.009  & Swope     \\
58887.69 & +33.49  & $B$    & 16.067               & 0.235  & $Swift$   \\
58893.3  & +39.1   & $B$    & 17.434               & 0.011  & Swope     \\
58894.32 & +40.12  & $B$    & 16.989               & 0.054  & Swope     \\
58895.43 & +41.23  & $B$    & 19.131               & 1.086  & Nickel    \\
58897.33 & +43.13  & $B$    & 16.875               & 0.012  & Swope     \\
58898.57 & +44.37  & $B$    & 16.285               & 0.202  & $Swift$   \\
58903.29 & +49.09  & $B$    & 17.427               & 0.016  & Swope     \\
58904.34 & +50.14  & $B$    & 17.58                & 0.014  & Swope     \\
58905.31 & +51.11  & $B$    & 17.564               & 0.008  & Swope     \\
58906.29 & +52.09  & $B$    & 17.613               & 0.017  & Swope     \\
58906.3  & +52.1   & $B$    & 17.599               & 0.008  & Swope     \\
58907.26 & +53.06  & $B$    & 16.335               & 0.188  & $Swift$   \\
58907.38 & +53.18  & $B$    & 17.554               & 0.016  & Swope     \\
58908.32 & +54.12  & $B$    & 17.559               & 0.017  & Swope     \\
58908.33 & +54.13  & $B$    & 17.581               & 0.011  & Swope     \\
58909.37 & +55.17  & $B$    & 17.649               & 0.011  & Swope     \\
58910.26 & +56.06  & $B$    & 17.562               & 0.016  & Swope     \\
58911.21 & +57.01  & $B$    & 17.655               & 0.016  & Swope     \\
58912.28 & +58.08  & $B$    & 17.669               & 0.016  & Swope     \\
58921.26 & +67.06  & $B$    & 17.332               & 0.095  & Swope     \\
58923.29 & +69.09  & $B$    & 17.239               & 0.023  & Swope     \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58954.16 & +99.96  & $B$    & 18.846               & 1.086  & Nickel    \\
58963.19 & +108.99 & $B$    & 18.354               & 1.086  & Nickel    \\
58856.31 & +2.11   & $g$    & 16.287               & 0.018  & LCO       \\
58856.33 & +2.13   & $g$    & 16.254               & 0.014  & LCO       \\
58856.33 & +2.13   & $g$    & 16.268               & 0.015  & LCO       \\
58856.35 & +2.15   & $g$    & 16.305               & 0.016  & LCO       \\
58856.37 & +2.17   & $g$    & 16.3                 & 0.021  & LCO       \\
58856.41 & +2.21   & $g$    & 16.014               & 0.017  & LCO       \\
58856.73 & +2.53   & $g$    & 16.039               & 0.012  & LCO       \\
58856.73 & +2.53   & $g$    & 16.02                & 0.013  & LCO       \\
58857.3  & +3.1    & $g$    & 15.799               & 0.013  & LCO       \\
58857.32 & +3.12   & $g$    & 15.821               & 0.013  & LCO       \\
58857.35 & +3.15   & $g$    & 15.858               & 0.014  & LCO       \\
58857.36 & +3.16   & $g$    & 15.683               & 0.113  & LCO       \\
58857.71 & +3.51   & $g$    & 15.684               & 0.017  & LCO       \\
58857.72 & +3.52   & $g$    & 15.645               & 0.016  & LCO       \\
58858.3  & +4.1    & $g$    & 15.337               & 0.012  & LCO       \\
58858.3  & +4.1    & $g$    & 15.416               & 0.01   & LCO       \\
58858.31 & +4.11   & $g$    & 15.401               & 0.01   & LCO       \\
58858.34 & +4.14   & $g$    & 15.355               & 0.012  & LCO       \\
58859.05 & +4.85   & $g$    & 15.103               & 0.01   & LCO       \\
58859.3  & +5.1    & $g$    & 14.993               & 0.01   & LCO       \\
58859.52 & +5.32   & $g$    & 14.916               & 0.028  & ZTF       \\
58859.69 & +5.49   & $g$    & 14.864               & 0.01   & LCO       \\
58860.05 & +5.85   & $g$    & 15.124               & 0.059  & LCO       \\
58860.05 & +5.85   & $g$    & 17.026               & 1.086  & LCO       \\
58860.05 & +5.85   & $g$    & 14.706               & 0.009  & LCO       \\
58860.07 & +5.87   & $g$    & 14.638               & 0.009  & LCO       \\
58860.07 & +5.87   & $g$    & 14.628               & 0.009  & LCO       \\
58861.05 & +6.85   & $g$    & 14.355               & 0.01   & LCO       \\
58861.29 & +7.09   & $g$    & 14.433               & 0.01   & LCO       \\
58861.35 & +7.15   & $g$    & 14.307               & 0.009  & LCO       \\
58861.35 & +7.15   & $g$    & 14.329               & 0.009  & LCO       \\
58861.68 & +7.48   & $g$    & 14.26                & 0.012  & LCO       \\
58862.36 & +8.16   & $g$    & 14.134               & 0.009  & LCO       \\
58862.36 & +8.16   & $g$    & 14.128               & 0.009  & LCO       \\
58862.53 & +8.33   & $g$    & 14.059               & 0.023  & Thacher   \\
58863.53 & +9.33   & $g$    & 13.044               & 0.017  & Thacher   \\
58864.34 & +10.14  & $g$    & 13.992               & 0.018  & Thacher   \\
58864.75 & +10.55  & $g$    & 14.05                & 0.009  & LCO       \\
58865.45 & +11.25  & $g$    & 14.048               & 0.018  & Thacher   \\
58866.3  & +12.1   & $g$    & 14.08                & 0.009  & LCO       \\
58866.32 & +12.12  & $g$    & 14.101               & 0.014  & Thacher   \\
58866.57 & +12.37  & $g$    & 14.093               & 0.004  & PS1       \\
58867.3  & +13.1   & $g$    & 14.296               & 0.009  & LCO       \\
58867.3  & +13.1   & $g$    & 14.208               & 0.015  & LCO       \\
58867.3  & +13.1   & $g$    & 14.208               & 0.015  & LCO       \\
58867.35 & +13.15  & $g$    & 14.201               & 0.015  & Thacher   \\
58867.4  & +13.2   & $g$    & 14.271               & 0.009  & LCO       \\
58867.4  & +13.2   & $g$    & 14.251               & 0.009  & LCO       \\
58867.44 & +13.24  & $g$    & 14.3                 & 0.03   & ZTF       \\
58868.27 & +14.07  & $g$    & 14.441               & 0.009  & LCO       \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58869.27 & +15.07  & $g$    & 14.583               & 0.009  & LCO       \\
58869.35 & +15.15  & $g$    & 14.654               & 0.004  & Swope     \\
58869.36 & +15.16  & $g$    & 14.584               & 0.009  & LCO       \\
58869.36 & +15.16  & $g$    & 14.577               & 0.009  & LCO       \\
58869.57 & +15.37  & $g$    & 14.576               & 0.005  & PS1       \\
58870.27 & +16.07  & $g$    & 14.864               & 0.01   & LCO       \\
58871.27 & +17.07  & $g$    & 15.096               & 0.011  & LCO       \\
58871.32 & +17.12  & $g$    & 15.004               & 0.01   & LCO       \\
58871.32 & +17.12  & $g$    & 15.0                 & 0.01   & LCO       \\
58871.33 & +17.13  & $g$    & 14.899               & 0.013  & Thacher   \\
58871.35 & +17.15  & $g$    & 14.995               & 0.003  & Swope     \\
58871.44 & +17.24  & $g$    & 15.03                & 0.024  & ZTF       \\
58872.29 & +18.09  & $g$    & 15.16                & 0.01   & LCO       \\
58872.33 & +18.13  & $g$    & 15.073               & 0.014  & Thacher   \\
58872.35 & +18.15  & $g$    & 15.21                & 0.004  & Swope     \\
58872.35 & +18.15  & $g$    & 15.086               & 0.013  & Swope     \\
58873.09 & +18.89  & $g$    & 15.224               & 0.01   & LCO       \\
58873.09 & +18.89  & $g$    & 15.273               & 0.011  & LCO       \\
58873.09 & +18.89  & $g$    & 15.235               & 0.01   & LCO       \\
58873.4  & +19.2   & $g$    & 15.312               & 0.017  & Thacher   \\
58874.28 & +20.08  & $g$    & 15.447               & 0.012  & LCO       \\
58874.29 & +20.09  & $g$    & 15.414               & 0.017  & Thacher   \\
58875.25 & +21.05  & $g$    & 15.68                & 0.012  & LCO       \\
58875.38 & +21.18  & $g$    & 15.659               & 0.008  & Swope     \\
58875.46 & +21.26  & $g$    & 15.676               & 0.025  & ZTF       \\
58876.03 & +21.83  & $g$    & 15.704               & 0.012  & LCO       \\
58876.03 & +21.83  & $g$    & 15.689               & 0.012  & LCO       \\
58876.29 & +22.09  & $g$    & 15.635               & 0.035  & Thacher   \\
58876.33 & +22.13  & $g$    & 15.837               & 0.036  & LCO       \\
58876.36 & +22.16  & $g$    & 15.779               & 0.007  & Swope     \\
58877.03 & +22.83  & $g$    & 15.829               & 0.013  & LCO       \\
58877.03 & +22.83  & $g$    & 15.848               & 0.013  & LCO       \\
58877.26 & +23.06  & $g$    & 15.913               & 0.016  & LCO       \\
58877.26 & +23.06  & $g$    & 15.874               & 0.028  & LCO       \\
58878.06 & +23.86  & $g$    & 16.895               & 1.086  & LCO       \\
58878.34 & +24.14  & $g$    & 16.023               & 0.013  & LCO       \\
58878.49 & +24.29  & $g$    & 16.039               & 0.024  & ZTF       \\
58879.08 & +24.88  & $g$    & 17.228               & 1.086  & LCO       \\
58880.12 & +25.92  & $g$    & 16.067               & 0.016  & LCO       \\
58880.12 & +25.92  & $g$    & 16.096               & 0.016  & LCO       \\
58880.28 & +26.08  & $g$    & 16.148               & 0.023  & Thacher   \\
58881.28 & +27.08  & $g$    & 16.223               & 0.021  & Thacher   \\
58881.46 & +27.26  & $g$    & 16.326               & 0.026  & ZTF       \\
58881.99 & +27.79  & $g$    & 16.258               & 0.016  & LCO       \\
58882.09 & +27.89  & $g$    & 16.28                & 0.016  & LCO       \\
58882.09 & +27.89  & $g$    & 16.326               & 0.017  & LCO       \\
58882.32 & +28.12  & $g$    & 16.396               & 0.007  & Swope     \\
58883.01 & +28.81  & $g$    & 18.139               & 1.086  & LCO       \\
58883.01 & +28.81  & $g$    & 16.378               & 0.02   & LCO       \\
58883.01 & +28.81  & $g$    & 16.388               & 0.019  & LCO       \\
58883.12 & +28.92  & $g$    & 16.322               & 0.016  & LCO       \\
58883.12 & +28.92  & $g$    & 16.346               & 0.016  & LCO       \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58883.38 & +29.18  & $g$    & 16.475               & 0.007  & Swope     \\
58883.99 & +29.79  & $g$    & 16.39                & 0.016  & LCO       \\
58884.0  & +29.8   & $g$    & 16.491               & 0.018  & LCO       \\
58884.37 & +30.17  & $g$    & 16.477               & 0.017  & LCO       \\
58884.37 & +30.17  & $g$    & 16.489               & 0.009  & Swope     \\
58884.37 & +30.17  & $g$    & 16.315               & 0.3    & LCO       \\
58884.37 & +30.17  & $g$    & 17.73                & 1.086  & LCO       \\
58884.44 & +30.24  & $g$    & 16.491               & 0.033  & ZTF       \\
58885.36 & +31.16  & $g$    & 16.559               & 0.011  & Swope     \\
58885.37 & +31.17  & $g$    & 16.472               & 0.023  & Thacher   \\
58885.38 & +31.18  & $g$    & 16.368               & 1.086  & Swope     \\
58886.28 & +32.08  & $g$    & 16.557               & 0.065  & Thacher   \\
58887.43 & +33.23  & $g$    & 16.608               & 0.043  & ZTF       \\
58890.28 & +36.08  & $g$    & 16.254               & 0.22   & Thacher   \\
58892.26 & +38.06  & $g$    & 16.686               & 0.042  & Thacher   \\
58892.38 & +38.18  & $g$    & 16.766               & 0.035  & ZTF       \\
58893.25 & +39.05  & $g$    & 16.636               & 0.018  & Thacher   \\
58893.29 & +39.09  & $g$    & 16.811               & 0.01   & Swope     \\
58894.25 & +40.05  & $g$    & 16.756               & 0.02   & Thacher   \\
58894.31 & +40.11  & $g$    & 16.821               & 0.009  & Swope     \\
58895.29 & +41.09  & $g$    & 16.844               & 0.009  & Swope     \\
58895.29 & +41.09  & $g$    & 17.04                & 1.086  & LCO       \\
58895.38 & +41.18  & $g$    & 16.816               & 0.028  & ZTF       \\
58896.29 & +42.09  & $g$    & 16.861               & 0.021  & Swope     \\
58897.31 & +43.11  & $g$    & 16.534               & 0.009  & Swope     \\
58898.24 & +44.04  & $g$    & 16.919               & 0.025  & Thacher   \\
58898.42 & +44.22  & $g$    & 16.893               & 0.036  & ZTF       \\
58899.23 & +45.03  & $g$    & 16.922               & 0.039  & Thacher   \\
58899.4  & +45.2   & $g$    & 16.916               & 0.037  & ZTF       \\
58900.34 & +46.14  & $g$    & 16.954               & 0.046  & Thacher   \\
58902.24 & +48.04  & $g$    & 17.019               & 1.086  & LCO       \\
58903.27 & +49.07  & $g$    & 16.984               & 0.013  & Swope     \\
58903.29 & +49.09  & $g$    & 16.81                & 0.029  & Thacher   \\
58903.36 & +49.16  & $g$    & 16.925               & 0.036  & ZTF       \\
58904.32 & +50.12  & $g$    & 16.996               & 0.01   & Swope     \\
58904.46 & +50.26  & $g$    & 16.972               & 0.049  & ZTF       \\
58905.29 & +51.09  & $g$    & 17.031               & 0.009  & Swope     \\
58905.31 & +51.11  & $g$    & 16.962               & 0.043  & ZTF       \\
58905.57 & +51.37  & $g$    & 16.405               & 0.102  & Thacher   \\
58906.28 & +52.08  & $g$    & 17.04                & 0.01   & Swope     \\
58907.36 & +53.16  & $g$    & 17.057               & 0.011  & Swope     \\
58908.31 & +54.11  & $g$    & 17.046               & 0.015  & Swope     \\
58908.31 & +54.11  & $g$    & 17.07                & 0.014  & Swope     \\
58908.34 & +54.14  & $g$    & 17.035               & 0.049  & ZTF       \\
58909.36 & +55.16  & $g$    & 17.138               & 0.01   & Swope     \\
58910.25 & +56.05  & $g$    & 17.148               & 0.013  & Swope     \\
58911.2  & +57.0   & $g$    & 17.15                & 0.014  & Swope     \\
58911.4  & +57.2   & $g$    & 17.165               & 0.044  & ZTF       \\
58912.27 & +58.07  & $g$    & 17.157               & 0.014  & Swope     \\
58913.33 & +59.13  & $g$    & 17.102               & 0.042  & ZTF       \\
58914.42 & +60.23  & $g$    & 17.244               & 0.046  & ZTF       \\
58915.44 & +61.24  & $g$    & 17.179               & 0.042  & ZTF       \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58919.14 & +64.94  & $g$    & 16.851               & 1.086  & LCO       \\
58919.14 & +64.94  & $g$    & 16.528               & 0.033  & LCO       \\
58923.14 & +68.94  & $g$    & 17.543               & 1.086  & LCO       \\
58929.5  & +75.3   & $g$    & 17.518               & 1.086  & LCO       \\
58929.5  & +75.3   & $g$    & 16.359               & 0.047  & LCO       \\
58935.64 & +81.44  & $g$    & 17.201               & 1.086  & LCO       \\
58935.64 & +81.44  & $g$    & 17.201               & 0.362  & LCO       \\
58939.34 & +85.14  & $g$    & 17.873               & 0.069  & ZTF       \\
58940.39 & +86.19  & $g$    & 17.759               & 0.068  & ZTF       \\
58943.46 & +89.26  & $g$    & 17.138               & 0.362  & LCO       \\
58943.46 & +89.26  & $g$    & 17.137               & 1.086  & LCO       \\
58952.44 & +98.24  & $g$    & 18.185               & 1.086  & LCO       \\
58959.34 & +105.14 & $g$    & 17.853               & 1.086  & LCO       \\
58962.23 & +108.03 & $g$    & 18.439               & 0.077  & ZTF       \\
58966.35 & +112.15 & $g$    & 16.811               & 1.086  & LCO       \\
58967.23 & +113.03 & $g$    & 18.608               & 0.103  & ZTF       \\
58974.11 & +119.91 & $g$    & 17.167               & 1.086  & LCO       \\
58980.76 & +126.56 & $g$    & 17.287               & 1.086  & LCO       \\
58988.32 & +134.12 & $g$    & 17.391               & 1.086  & LCO       \\
58996.5  & +142.3  & $g$    & 17.503               & 1.086  & LCO       \\
59002.75 & +148.55 & $g$    & 18.9                 & 1.086  & LCO       \\
59007.71 & +153.51 & $g$    & 18.616               & 1.086  & LCO       \\
59014.8  & +160.6  & $g$    & 19.206               & 1.086  & LCO       \\
59026.35 & +172.15 & $g$    & 17.31                & 1.086  & LCO       \\
59032.34 & +178.14 & $g$    & 20.351               & 1.086  & LCO       \\
59038.72 & +184.52 & $g$    & 19.725               & 1.086  & LCO       \\
59202.09 & +347.89 & $g$    & 18.595               & 1.086  & LCO       \\
59208.07 & +353.87 & $g$    & 18.397               & 1.086  & LCO       \\
59214.05 & +359.85 & $g$    & 17.82                & 1.086  & LCO       \\
59220.37 & +366.17 & $g$    & 18.414               & 1.086  & LCO       \\
59226.11 & +371.91 & $g$    & 17.649               & 1.086  & LCO       \\
59227.71 & +373.51 & $g$    & 18.809               & 1.086  & LCO       \\
59232.37 & +378.17 & $g$    & 17.354               & 1.086  & LCO       \\
59236.06 & +381.86 & $g$    & 18.162               & 1.086  & LCO       \\
59245.42 & +391.22 & $g$    & 18.691               & 1.086  & LCO       \\
59252.06 & +397.86 & $g$    & 18.123               & 1.086  & LCO       \\
59257.33 & +403.13 & $g$    & 19.219               & 1.086  & LCO       \\
59262.22 & +408.02 & $g$    & 18.373               & 1.086  & LCO       \\
59267.12 & +412.92 & $g$    & 17.455               & 1.086  & LCO       \\
58856.46 & +2.26   & $V$    & 16.122               & 0.245  & $Swift$   \\
58856.8  & +2.6    & $V$    & 16.211               & 0.263  & $Swift$   \\
58857.45 & +3.25   & $V$    & 15.781               & 0.195  & $Swift$   \\
58858.85 & +4.65   & $V$    & 15.222               & 0.142  & $Swift$   \\
58860.38 & +6.18   & $V$    & 14.66                & 0.11   & $Swift$   \\
58861.25 & +7.05   & $V$    & 14.329               & 0.097  & $Swift$   \\
58869.35 & +15.15  & $V$    & 14.199               & 0.003  & Swope     \\
58869.36 & +15.16  & $V$    & 14.043               & 0.011  & LCO       \\
58870.32 & +16.12  & $V$    & 14.296               & 0.005  & Swope     \\
58870.32 & +16.12  & $V$    & 14.231               & 0.014  & Swope     \\
58871.31 & +17.11  & $V$    & 14.289               & 0.011  & LCO       \\
58871.36 & +17.16  & $V$    & 14.525               & 0.003  & Swope     \\
58872.36 & +18.16  & $V$    & 14.698               & 0.002  & Swope     \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58873.09 & +18.89  & $V$    & 17.928               & 1.086  & LCO       \\
58875.38 & +21.18  & $V$    & 15.089               & 0.006  & Swope     \\
58876.37 & +22.17  & $V$    & 15.316               & 0.004  & Swope     \\
58877.19 & +22.99  & $V$    & 15.207               & 0.152  & $Swift$   \\
58878.06 & +23.86  & $V$    & 16.157               & 1.086  & LCO       \\
58879.08 & +24.88  & $V$    & 16.023               & 1.086  & LCO       \\
58880.12 & +25.92  & $V$    & 17.259               & 1.086  & LCO       \\
58880.44 & +26.24  & $V$    & 18.163               & 1.086  & Nickel    \\
58882.33 & +28.13  & $V$    & 15.965               & 0.005  & Swope     \\
58883.12 & +28.92  & $V$    & 15.663               & 0.016  & LCO       \\
58883.38 & +29.18  & $V$    & 16.075               & 0.006  & Swope     \\
58884.37 & +30.17  & $V$    & 16.028               & 0.008  & Swope     \\
58885.37 & +31.17  & $V$    & 16.128               & 0.009  & Swope     \\
58887.68 & +33.48  & $V$    & 15.572               & 0.174  & $Swift$   \\
58893.3  & +39.1   & $V$    & 16.523               & 0.009  & Swope     \\
58894.32 & +40.12  & $V$    & 16.571               & 0.009  & Swope     \\
58895.3  & +41.1   & $V$    & 16.514               & 0.01   & Swope     \\
58895.43 & +41.23  & $V$    & 19.074               & 1.086  & Nickel    \\
58895.44 & +41.24  & $V$    & 18.828               & 1.086  & Nickel    \\
58896.3  & +42.1   & $V$    & 16.482               & 0.014  & Swope     \\
58897.32 & +43.12  & $V$    & 16.203               & 0.112  & Swope     \\
58898.57 & +44.37  & $V$    & 15.803               & 0.204  & $Swift$   \\
58899.32 & +45.12  & $V$    & 18.939               & 1.086  & Nickel    \\
58900.38 & +46.18  & $V$    & 18.582               & 1.086  & Nickel    \\
58903.28 & +49.08  & $V$    & 16.668               & 0.013  & Swope     \\
58904.34 & +50.14  & $V$    & 16.804               & 0.01   & Swope     \\
58904.35 & +50.15  & $V$    & 18.479               & 1.086  & Nickel    \\
58905.3  & +51.1   & $V$    & 16.806               & 0.006  & Swope     \\
58906.29 & +52.09  & $V$    & 16.832               & 0.006  & Swope     \\
58907.25 & +53.05  & $V$    & 15.936               & 0.217  & $Swift$   \\
58907.37 & +53.17  & $V$    & 16.789               & 0.01   & Swope     \\
58908.32 & +54.12  & $V$    & 16.809               & 0.015  & Swope     \\
58908.32 & +54.12  & $V$    & 16.788               & 0.01   & Swope     \\
58909.37 & +55.17  & $V$    & 16.907               & 0.009  & Swope     \\
58910.26 & +56.06  & $V$    & 16.855               & 0.011  & Swope     \\
58911.21 & +57.01  & $V$    & 16.862               & 0.01   & Swope     \\
58912.28 & +58.08  & $V$    & 16.984               & 0.011  & Swope     \\
58921.26 & +67.06  & $V$    & 16.905               & 0.036  & Swope     \\
58923.29 & +69.09  & $V$    & 16.745               & 0.015  & Swope     \\
58963.2  & +109.0  & $V$    & 17.992               & 1.086  & Nickel    \\
58855.54 & +1.34   & $r$    & 17.28                & 0.056  & ZTF       \\
58856.31 & +2.11   & $r$    & 16.312               & 0.02   & LCO       \\
58856.31 & +2.11   & $r$    & 16.843               & 1.086  & LCO       \\
58856.33 & +2.13   & $r$    & 16.481               & 0.018  & LCO       \\
58856.33 & +2.13   & $r$    & 16.483               & 0.017  & LCO       \\
58856.37 & +2.17   & $r$    & 15.871               & 0.02   & LCO       \\
58856.41 & +2.21   & $r$    & 16.773               & 1.086  & LCO       \\
58856.41 & +2.21   & $r$    & 16.945               & 0.283  & LCO       \\
58856.41 & +2.21   & $r$    & 16.121               & 0.019  & LCO       \\
58856.7  & +2.5    & $r$    & 16.246               & 0.025  & LCO       \\
58856.74 & +2.54   & $r$    & 16.069               & 0.016  & LCO       \\
58856.74 & +2.54   & $r$    & 16.074               & 0.016  & LCO       \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58857.3  & +3.1    & $r$    & 15.524               & 0.014  & LCO       \\
58857.3  & +3.1    & $r$    & 15.775               & 0.013  & LCO       \\
58857.3  & +3.1    & $r$    & 17.172               & 1.086  & LCO       \\
58857.32 & +3.12   & $r$    & 17.359               & 1.086  & LCO       \\
58857.32 & +3.12   & $r$    & 15.841               & 0.012  & LCO       \\
58857.35 & +3.15   & $r$    & 17.56                & 1.086  & LCO       \\
58857.35 & +3.15   & $r$    & 15.808               & 0.012  & LCO       \\
58857.37 & +3.17   & $r$    & 15.989               & 0.177  & LCO       \\
58857.72 & +3.52   & $r$    & 15.57                & 0.014  & LCO       \\
58857.72 & +3.52   & $r$    & 15.422               & 0.014  & LCO       \\
58858.3  & +4.1    & $r$    & 15.291               & 0.009  & LCO       \\
58858.3  & +4.1    & $r$    & 15.2                 & 0.029  & LCO       \\
58858.3  & +4.1    & $r$    & 15.302               & 0.009  & LCO       \\
58858.31 & +4.11   & $r$    & 15.324               & 0.009  & LCO       \\
58858.34 & +4.14   & $r$    & 15.242               & 0.011  & LCO       \\
58859.05 & +4.85   & $r$    & 15.13                & 0.009  & LCO       \\
58859.3  & +5.1    & $r$    & 14.907               & 0.009  & LCO       \\
58859.48 & +5.28   & $r$    & 14.769               & 0.033  & ZTF       \\
58859.69 & +5.49   & $r$    & 14.786               & 0.009  & LCO       \\
58860.05 & +5.85   & $r$    & 14.657               & 0.008  & LCO       \\
58860.08 & +5.88   & $r$    & 14.641               & 0.008  & LCO       \\
58860.08 & +5.88   & $r$    & 14.652               & 0.008  & LCO       \\
58860.42 & +6.22   & $r$    & -13.051              & 1.086  & LCO       \\
58861.05 & +6.85   & $r$    & 14.372               & 0.008  & LCO       \\
58861.29 & +7.09   & $r$    & 14.327               & 0.008  & LCO       \\
58861.35 & +7.15   & $r$    & 14.382               & 0.008  & LCO       \\
58861.35 & +7.15   & $r$    & 14.333               & 0.008  & LCO       \\
58861.68 & +7.48   & $r$    & 14.305               & 0.009  & LCO       \\
58862.36 & +8.16   & $r$    & 14.197               & 0.008  & LCO       \\
58862.37 & +8.17   & $r$    & 14.211               & 0.008  & LCO       \\
58864.31 & +10.11  & $r$    & 13.904               & 0.033  & LCO       \\
58864.34 & +10.14  & $r$    & 13.95                & 0.015  & Thacher   \\
58864.75 & +10.55  & $r$    & 13.951               & 0.008  & LCO       \\
58864.75 & +10.55  & $r$    & 13.874               & 0.011  & LCO       \\
58864.75 & +10.55  & $r$    & 13.874               & 0.011  & LCO       \\
58865.46 & +11.26  & $r$    & 13.887               & 0.018  & Thacher   \\
58866.31 & +12.11  & $r$    & 13.828               & 0.009  & LCO       \\
58866.32 & +12.12  & $r$    & 13.902               & 0.012  & Thacher   \\
58867.3  & +13.1   & $r$    & 13.892               & 0.008  & LCO       \\
58867.35 & +13.15  & $r$    & 13.902               & 0.013  & Thacher   \\
58867.4  & +13.2   & $r$    & 13.887               & 0.008  & LCO       \\
58867.4  & +13.2   & $r$    & 13.922               & 0.008  & LCO       \\
58867.48 & +13.28  & $r$    & 13.86                & 0.02   & ZTF       \\
58868.27 & +14.07  & $r$    & 13.828               & 0.008  & LCO       \\
58868.27 & +14.07  & $r$    & 14.01                & 0.008  & LCO       \\
58868.27 & +14.07  & $r$    & 13.828               & 0.008  & LCO       \\
58869.27 & +15.07  & $r$    & 14.148               & 0.008  & LCO       \\
58869.35 & +15.15  & $r$    & 13.953               & 0.003  & Swope     \\
58869.35 & +15.15  & $r$    & 14.079               & 0.005  & Swope     \\
58869.36 & +15.16  & $r$    & 13.999               & 0.008  & LCO       \\
58869.36 & +15.16  & $r$    & 14.008               & 0.008  & LCO       \\
58869.57 & +15.37  & $r$    & 13.956               & 0.003  & PS1       \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58870.27 & +16.07  & $r$    & 14.33                & 0.008  & LCO       \\
58870.31 & +16.11  & $r$    & 14.015               & 0.004  & Swope     \\
58871.27 & +17.07  & $r$    & 14.332               & 0.008  & LCO       \\
58871.32 & +17.12  & $r$    & 14.246               & 0.008  & LCO       \\
58871.32 & +17.12  & $r$    & 14.256               & 0.009  & LCO       \\
58871.32 & +17.12  & $r$    & 14.188               & 0.012  & LCO       \\
58871.34 & +17.14  & $r$    & 14.209               & 0.011  & Thacher   \\
58871.35 & +17.15  & $r$    & 14.121               & 0.003  & Swope     \\
58871.5  & +17.3   & $r$    & 14.17                & 0.035  & ZTF       \\
58872.29 & +18.09  & $r$    & 14.286               & 0.008  & LCO       \\
58872.33 & +18.13  & $r$    & 14.324               & 0.014  & Thacher   \\
58872.35 & +18.15  & $r$    & 14.388               & 0.002  & Swope     \\
58873.09 & +18.89  & $r$    & 14.421               & 0.009  & LCO       \\
58873.1  & +18.9   & $r$    & 14.467               & 0.009  & LCO       \\
58873.1  & +18.9   & $r$    & 14.49                & 0.009  & LCO       \\
58873.4  & +19.2   & $r$    & 14.422               & 0.012  & Thacher   \\
58874.28 & +20.08  & $r$    & 14.548               & 0.009  & LCO       \\
58874.29 & +20.09  & $r$    & 14.584               & 0.017  & Thacher   \\
58874.37 & +20.17  & $r$    & 14.607               & 0.004  & Swope     \\
58875.26 & +21.06  & $r$    & 14.792               & 0.009  & LCO       \\
58875.37 & +21.17  & $r$    & 14.662               & 0.004  & Swope     \\
58875.52 & +21.32  & $r$    & 14.677               & 0.025  & ZTF       \\
58876.03 & +21.83  & $r$    & 14.85                & 0.009  & LCO       \\
58876.03 & +21.83  & $r$    & 14.869               & 0.01   & LCO       \\
58876.29 & +22.09  & $r$    & 14.781               & 0.023  & Thacher   \\
58876.34 & +22.14  & $r$    & 14.95                & 0.013  & LCO       \\
58876.36 & +22.16  & $r$    & 14.821               & 0.005  & Swope     \\
58877.03 & +22.83  & $r$    & 18.286               & 1.086  & LCO       \\
58877.03 & +22.83  & $r$    & 14.949               & 0.01   & LCO       \\
58877.03 & +22.83  & $r$    & 14.966               & 0.01   & LCO       \\
58877.26 & +23.06  & $r$    & 15.011               & 0.012  & LCO       \\
58877.26 & +23.06  & $r$    & 14.976               & 0.012  & LCO       \\
58878.28 & +24.08  & $r$    & 14.926               & 0.023  & Thacher   \\
58878.34 & +24.14  & $r$    & 15.156               & 0.009  & LCO       \\
58878.36 & +24.16  & $r$    & 15.057               & 0.023  & ZTF       \\
58880.12 & +25.92  & $r$    & 15.345               & 0.013  & LCO       \\
58880.12 & +25.92  & $r$    & 15.291               & 0.014  & LCO       \\
58880.12 & +25.92  & $r$    & 17.633               & 1.086  & LCO       \\
58880.29 & +26.09  & $r$    & 15.356               & 0.016  & Thacher   \\
58880.44 & +26.24  & $r$    & 18.403               & 1.086  & Nickel    \\
58881.28 & +27.08  & $r$    & 15.439               & 0.014  & Thacher   \\
58881.54 & +27.34  & $r$    & 15.391               & 0.033  & ZTF       \\
58882.0  & +27.8   & $r$    & 15.596               & 0.012  & LCO       \\
58882.09 & +27.89  & $r$    & 15.531               & 0.012  & LCO       \\
58882.09 & +27.89  & $r$    & 15.532               & 0.012  & LCO       \\
58882.32 & +28.12  & $r$    & 15.658               & 0.007  & Swope     \\
58882.32 & +28.12  & $r$    & 15.636               & 0.005  & Swope     \\
58883.01 & +28.81  & $r$    & 15.565               & 0.015  & LCO       \\
58883.12 & +28.92  & $r$    & 15.672               & 0.012  & LCO       \\
58883.12 & +28.92  & $r$    & 15.612               & 0.012  & LCO       \\
58883.37 & +29.17  & $r$    & 15.728               & 0.005  & Swope     \\
58884.0  & +29.8   & $r$    & 15.747               & 0.014  & LCO       \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58884.0  & +29.8   & $r$    & 15.719               & 0.015  & LCO       \\
58884.37 & +30.17  & $r$    & 18.531               & 1.086  & LCO       \\
58884.37 & +30.17  & $r$    & 15.747               & 0.012  & LCO       \\
58884.37 & +30.17  & $r$    & 15.646               & 0.007  & Swope     \\
58884.52 & +30.32  & $r$    & 15.63                & 0.027  & ZTF       \\
58885.35 & +31.15  & $r$    & 15.759               & 0.006  & Swope     \\
58886.28 & +32.08  & $r$    & 15.834               & 0.023  & Thacher   \\
58887.52 & +33.32  & $r$    & 15.836               & 0.029  & ZTF       \\
58890.28 & +36.08  & $r$    & 15.936               & 0.056  & Thacher   \\
58892.27 & +38.07  & $r$    & 16.183               & 0.024  & Thacher   \\
58892.32 & +38.12  & $r$    & 16.089               & 0.032  & ZTF       \\
58893.25 & +39.05  & $r$    & 16.221               & 0.017  & Thacher   \\
58893.29 & +39.09  & $r$    & 16.306               & 0.006  & Swope     \\
58894.26 & +40.06  & $r$    & 16.33                & 0.015  & Thacher   \\
58894.31 & +40.11  & $r$    & 16.314               & 0.006  & Swope     \\
58895.24 & +41.04  & $r$    & 16.884               & 0.255  & Swope     \\
58895.28 & +41.08  & $r$    & 16.24                & 0.009  & Swope     \\
58895.29 & +41.09  & $r$    & 16.717               & 1.086  & LCO       \\
58895.43 & +41.23  & $r$    & 16.316               & 0.166  & Nickel    \\
58895.44 & +41.24  & $r$    & 19.337               & 1.086  & Nickel    \\
58895.44 & +41.24  & $r$    & 16.182               & 0.034  & ZTF       \\
58896.29 & +42.09  & $r$    & 16.303               & 0.01   & Swope     \\
58897.31 & +43.11  & $r$    & 16.244               & 0.075  & Swope     \\
58897.31 & +43.11  & $r$    & 16.479               & 0.014  & Swope     \\
58898.24 & +44.04  & $r$    & 16.494               & 0.018  & Thacher   \\
58898.37 & +44.17  & $r$    & 16.301               & 0.035  & ZTF       \\
58899.23 & +45.03  & $r$    & 16.379               & 0.028  & Thacher   \\
58899.44 & +45.24  & $r$    & 16.38                & 0.032  & ZTF       \\
58900.34 & +46.14  & $r$    & 16.434               & 0.018  & Thacher   \\
58900.38 & +46.18  & $r$    & 16.457               & 0.304  & Nickel    \\
58900.44 & +46.24  & $r$    & 16.393               & 0.049  & ZTF       \\
58901.42 & +47.22  & $r$    & 16.428               & 0.056  & ZTF       \\
58902.24 & +48.04  & $r$    & 16.867               & 1.086  & LCO       \\
58902.26 & +48.06  & $r$    & 16.343               & 0.025  & Thacher   \\
58903.27 & +49.07  & $r$    & 16.573               & 0.023  & Swope     \\
58903.27 & +49.07  & $r$    & 16.487               & 0.01   & Swope     \\
58903.29 & +49.09  & $r$    & 16.573               & 0.025  & Thacher   \\
58904.32 & +50.12  & $r$    & 16.649               & 0.021  & Swope     \\
58904.32 & +50.12  & $r$    & 16.522               & 0.01   & Swope     \\
58904.35 & +50.15  & $r$    & 19.065               & 1.086  & Nickel    \\
58904.47 & +50.27  & $r$    & 16.497               & 0.028  & ZTF       \\
58905.28 & +51.08  & $r$    & 16.556               & 0.006  & Swope     \\
58905.28 & +51.08  & $r$    & 16.67                & 0.013  & Swope     \\
58905.57 & +51.37  & $r$    & 16.604               & 0.061  & Thacher   \\
58906.27 & +52.07  & $r$    & 16.568               & 0.006  & Swope     \\
58907.36 & +53.16  & $r$    & 16.672               & 0.008  & Swope     \\
58908.3  & +54.1   & $r$    & 16.739               & 0.008  & Swope     \\
58908.3  & +54.1   & $r$    & 16.783               & 0.012  & Swope     \\
58908.45 & +54.25  & $r$    & 16.638               & 0.042  & ZTF       \\
58909.35 & +55.15  & $r$    & 16.699               & 0.008  & Swope     \\
58910.16 & +55.96  & $r$    & 17.648               & 1.086  & LCO       \\
58910.24 & +56.04  & $r$    & 16.722               & 0.011  & Swope     \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58911.2  & +57.0   & $r$    & 16.74                & 0.008  & Swope     \\
58911.45 & +57.25  & $r$    & 16.721               & 0.039  & ZTF       \\
58912.27 & +58.07  & $r$    & 16.515               & 0.114  & Swope     \\
58912.45 & +58.25  & $r$    & 16.809               & 0.046  & ZTF       \\
58913.44 & +59.25  & $r$    & 16.824               & 0.046  & ZTF       \\
58914.27 & +60.07  & $r$    & 17.503               & 1.086  & LCO       \\
58915.4  & +61.2   & $r$    & 16.895               & 0.046  & ZTF       \\
58919.14 & +64.94  & $r$    & 16.736               & 1.086  & LCO       \\
58923.14 & +68.94  & $r$    & 17.568               & 1.086  & LCO       \\
58929.5  & +75.3   & $r$    & 17.344               & 1.086  & LCO       \\
58929.5  & +75.3   & $r$    & 13.408               & 1.086  & LCO       \\
58935.64 & +81.44  & $r$    & 16.847               & 1.086  & LCO       \\
58935.64 & +81.44  & $r$    & 16.847               & 0.362  & LCO       \\
58936.41 & +82.21  & $r$    & 17.594               & 0.058  & ZTF       \\
58942.51 & +88.31  & $r$    & 17.547               & 0.039  & PS1       \\
58943.46 & +89.26  & $r$    & 16.489               & 0.362  & LCO       \\
58943.46 & +89.26  & $r$    & 16.49                & 1.086  & LCO       \\
58952.44 & +98.24  & $r$    & 18.076               & 1.086  & LCO       \\
58954.18 & +99.98  & $r$    & 19.888               & 1.086  & Nickel    \\
58959.34 & +105.14 & $r$    & 17.86                & 1.086  & LCO       \\
58963.21 & +109.01 & $r$    & 19.444               & 1.086  & Nickel    \\
58965.29 & +111.09 & $r$    & 18.513               & 0.074  & ZTF       \\
58966.35 & +112.15 & $r$    & 16.915               & 1.086  & LCO       \\
58974.11 & +119.91 & $r$    & 17.159               & 1.086  & LCO       \\
58976.42 & +122.22 & $r$    & 18.29                & 0.157  & PS1       \\
58980.76 & +126.56 & $r$    & 17.186               & 1.086  & LCO       \\
58988.32 & +134.12 & $r$    & 17.241               & 1.086  & LCO       \\
58996.5  & +142.3  & $r$    & 17.511               & 1.086  & LCO       \\
59002.75 & +148.55 & $r$    & 18.868               & 1.086  & LCO       \\
59007.71 & +153.51 & $r$    & 18.827               & 1.086  & LCO       \\
59014.8  & +160.6  & $r$    & 19.062               & 1.086  & LCO       \\
59032.34 & +178.14 & $r$    & 20.364               & 1.086  & LCO       \\
59038.72 & +184.52 & $r$    & 19.669               & 1.086  & LCO       \\
59202.1  & +347.9  & $r$    & 18.793               & 1.086  & LCO       \\
59208.07 & +353.87 & $r$    & 18.553               & 1.086  & LCO       \\
59214.05 & +359.85 & $r$    & 18.295               & 1.086  & LCO       \\
59220.37 & +366.17 & $r$    & 18.209               & 1.086  & LCO       \\
59226.11 & +371.91 & $r$    & 17.922               & 1.086  & LCO       \\
59227.72 & +373.52 & $r$    & 18.699               & 1.086  & LCO       \\
59232.38 & +378.18 & $r$    & 16.923               & 1.086  & LCO       \\
59236.06 & +381.86 & $r$    & 18.111               & 1.086  & LCO       \\
59245.42 & +391.22 & $r$    & 18.625               & 1.086  & LCO       \\
59252.06 & +397.86 & $r$    & 18.136               & 1.086  & LCO       \\
59257.33 & +403.13 & $r$    & 19.168               & 1.086  & LCO       \\
59262.23 & +408.03 & $r$    & 18.583               & 1.086  & LCO       \\
59267.12 & +412.92 & $r$    & 17.345               & 1.086  & LCO       \\
58873.25 & +19.05  & $G$    & 14.58                & 0.2    & Gaia      \\
58856.31 & +2.11   & $i$    & 17.755               & 0.114  & LCO       \\
58856.34 & +2.14   & $i$    & 16.805               & 0.026  & LCO       \\
58856.34 & +2.14   & $i$    & 16.712               & 0.025  & LCO       \\
58856.37 & +2.17   & $i$    & 16.387               & 0.035  & LCO       \\
58856.37 & +2.17   & $i$    & 16.208               & 1.086  & LCO       \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58856.41 & +2.21   & $i$    & 16.362               & 0.025  & LCO       \\
58856.7  & +2.5    & $i$    & 15.986               & 0.059  & LCO       \\
58856.7  & +2.5    & $i$    & 14.922               & 1.086  & LCO       \\
58856.7  & +2.5    & $i$    & 15.352               & 0.04   & LCO       \\
58856.74 & +2.54   & $i$    & 16.323               & 0.052  & LCO       \\
58856.74 & +2.54   & $i$    & 16.304               & 0.017  & LCO       \\
58857.3  & +3.1    & $i$    & 16.171               & 0.019  & LCO       \\
58857.32 & +3.12   & $i$    & 16.058               & 0.016  & LCO       \\
58857.35 & +3.15   & $i$    & 15.983               & 0.014  & LCO       \\
58857.72 & +3.52   & $i$    & 16.975               & 1.086  & LCO       \\
58857.72 & +3.52   & $i$    & 15.629               & 0.022  & LCO       \\
58857.72 & +3.52   & $i$    & 15.544               & 0.02   & LCO       \\
58858.3  & +4.1    & $i$    & 15.52                & 0.01   & LCO       \\
58858.3  & +4.1    & $i$    & 15.524               & 0.01   & LCO       \\
58858.31 & +4.11   & $i$    & 15.551               & 0.011  & LCO       \\
58858.34 & +4.14   & $i$    & 15.415               & 0.013  & LCO       \\
58859.05 & +4.85   & $i$    & 15.207               & 0.01   & LCO       \\
58859.3  & +5.1    & $i$    & 15.118               & 0.009  & LCO       \\
58859.69 & +5.49   & $i$    & 14.989               & 0.01   & LCO       \\
58860.05 & +5.85   & $i$    & 14.818               & 0.009  & LCO       \\
58860.08 & +5.88   & $i$    & 14.868               & 0.007  & LCO       \\
58860.08 & +5.88   & $i$    & 14.833               & 0.007  & LCO       \\
58861.05 & +6.85   & $i$    & 14.515               & 0.009  & LCO       \\
58861.05 & +6.85   & $i$    & 14.577               & 0.009  & LCO       \\
58861.29 & +7.09   & $i$    & 14.545               & 0.008  & LCO       \\
58861.35 & +7.15   & $i$    & 14.619               & 0.008  & LCO       \\
58861.35 & +7.15   & $i$    & 14.588               & 0.007  & LCO       \\
58861.69 & +7.49   & $i$    & 14.239               & 0.012  & LCO       \\
58861.69 & +7.49   & $i$    & 16.09                & 1.086  & LCO       \\
58861.69 & +7.49   & $i$    & 14.438               & 0.009  & LCO       \\
58862.37 & +8.17   & $i$    & 14.318               & 0.007  & LCO       \\
58862.37 & +8.17   & $i$    & 14.313               & 0.007  & LCO       \\
58862.53 & +8.33   & $i$    & 14.261               & 0.021  & Thacher   \\
58864.31 & +10.11  & $i$    & 14.104               & 0.028  & LCO       \\
58864.34 & +10.14  & $i$    & 14.074               & 0.015  & Thacher   \\
58864.76 & +10.56  & $i$    & 14.132               & 0.008  & LCO       \\
58865.46 & +11.26  & $i$    & 13.999               & 0.042  & Thacher   \\
58866.31 & +12.11  & $i$    & 13.971               & 0.009  & LCO       \\
58866.33 & +12.13  & $i$    & 14.025               & 0.013  & Thacher   \\
58866.56 & +12.36  & $i$    & 14.001               & 0.005  & PS1       \\
58867.3  & +13.1   & $i$    & 14.08                & 0.008  & LCO       \\
58867.35 & +13.15  & $i$    & 14.061               & 0.016  & Thacher   \\
58867.4  & +13.2   & $i$    & 14.029               & 0.007  & LCO       \\
58867.4  & +13.2   & $i$    & 14.002               & 0.007  & LCO       \\
58868.28 & +14.08  & $i$    & 14.237               & 0.007  & LCO       \\
58869.27 & +15.07  & $i$    & 14.214               & 0.007  & LCO       \\
58869.35 & +15.15  & $i$    & 14.09                & 0.016  & Swope     \\
58869.36 & +15.16  & $i$    & 14.176               & 0.008  & LCO       \\
58869.36 & +15.16  & $i$    & 14.155               & 0.008  & LCO       \\
58870.27 & +16.07  & $i$    & 14.488               & 0.008  & LCO       \\
58870.32 & +16.12  & $i$    & 14.214               & 0.006  & Swope     \\
58870.32 & +16.12  & $i$    & 14.122               & 0.009  & Swope     \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58871.32 & +17.12  & $i$    & 14.367               & 0.009  & LCO       \\
58871.32 & +17.12  & $i$    & 14.296               & 0.009  & LCO       \\
58871.34 & +17.14  & $i$    & 14.299               & 0.012  & Thacher   \\
58871.35 & +17.15  & $i$    & 14.27                & 0.005  & Swope     \\
58872.29 & +18.09  & $i$    & 14.304               & 0.011  & LCO       \\
58872.29 & +18.09  & $i$    & 14.391               & 0.008  & LCO       \\
58872.29 & +18.09  & $i$    & 14.304               & 0.011  & LCO       \\
58872.33 & +18.13  & $i$    & 14.364               & 0.014  & Thacher   \\
58872.35 & +18.15  & $i$    & 14.52                & 0.004  & Swope     \\
58873.09 & +18.89  & $i$    & 14.536               & 0.008  & LCO       \\
58873.1  & +18.9   & $i$    & 14.457               & 0.008  & LCO       \\
58873.1  & +18.9   & $i$    & 14.467               & 0.009  & LCO       \\
58873.4  & +19.2   & $i$    & 14.482               & 0.011  & Thacher   \\
58874.29 & +20.09  & $i$    & 16.856               & 1.086  & LCO       \\
58874.29 & +20.09  & $i$    & 14.578               & 0.015  & Thacher   \\
58874.29 & +20.09  & $i$    & 14.602               & 0.009  & LCO       \\
58874.29 & +20.09  & $i$    & 14.766               & 0.073  & LCO       \\
58875.26 & +21.06  & $i$    & 14.802               & 0.009  & LCO       \\
58875.38 & +21.18  & $i$    & 14.702               & 0.005  & Swope     \\
58876.03 & +21.83  & $i$    & 14.849               & 0.009  & LCO       \\
58876.03 & +21.83  & $i$    & 14.844               & 0.009  & LCO       \\
58876.29 & +22.09  & $i$    & 14.631               & 0.025  & Thacher   \\
58876.34 & +22.14  & $i$    & 14.842               & 0.018  & LCO       \\
58876.36 & +22.16  & $i$    & 14.863               & 0.006  & Swope     \\
58877.03 & +22.83  & $i$    & 14.99                & 0.01   & LCO       \\
58877.03 & +22.83  & $i$    & 14.947               & 0.01   & LCO       \\
58877.27 & +23.07  & $i$    & 14.936               & 0.015  & LCO       \\
58878.07 & +23.87  & $i$    & 14.992               & 0.013  & LCO       \\
58878.07 & +23.87  & $i$    & 14.994               & 0.011  & LCO       \\
58878.07 & +23.87  & $i$    & 15.394               & 1.086  & LCO       \\
58878.29 & +24.09  & $i$    & 15.007               & 0.021  & Thacher   \\
58878.34 & +24.14  & $i$    & 15.079               & 0.01   & LCO       \\
58880.12 & +25.92  & $i$    & 15.323               & 0.016  & LCO       \\
58880.12 & +25.92  & $i$    & 15.287               & 0.014  & LCO       \\
58880.29 & +26.09  & $i$    & 15.304               & 0.017  & Thacher   \\
58880.44 & +26.24  & $i$    & 17.579               & 1.086  & Nickel    \\
58881.28 & +27.08  & $i$    & 15.403               & 0.015  & Thacher   \\
58882.0  & +27.8   & $i$    & 18.48                & 1.086  & LCO       \\
58882.0  & +27.8   & $i$    & 15.433               & 0.094  & LCO       \\
58882.0  & +27.8   & $i$    & 15.495               & 0.012  & LCO       \\
58882.09 & +27.89  & $i$    & 15.553               & 0.013  & LCO       \\
58882.09 & +27.89  & $i$    & 15.524               & 0.013  & LCO       \\
58882.32 & +28.12  & $i$    & 15.621               & 0.008  & Swope     \\
58883.12 & +28.92  & $i$    & 15.584               & 0.014  & LCO       \\
58883.12 & +28.92  & $i$    & 15.551               & 0.014  & LCO       \\
58883.37 & +29.17  & $i$    & 15.722               & 0.009  & Swope     \\
58884.0  & +29.8   & $i$    & 15.647               & 0.014  & LCO       \\
58884.0  & +29.8   & $i$    & 15.683               & 0.015  & LCO       \\
58884.37 & +30.17  & $i$    & 15.458               & 0.017  & Swope     \\
58884.37 & +30.17  & $i$    & 15.737               & 0.014  & LCO       \\
58885.35 & +31.15  & $i$    & 15.773               & 0.011  & Swope     \\
58886.28 & +32.08  & $i$    & 15.805               & 0.024  & Thacher   \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
58890.28 & +36.08  & $i$    & 15.864               & 0.048  & Thacher   \\
58892.27 & +38.07  & $i$    & 16.13                & 0.028  & Thacher   \\
58893.25 & +39.05  & $i$    & 16.141               & 0.018  & Thacher   \\
58893.29 & +39.09  & $i$    & 16.208               & 0.01   & Swope     \\
58894.26 & +40.06  & $i$    & 16.267               & 0.021  & Thacher   \\
58894.31 & +40.11  & $i$    & 16.321               & 0.01   & Swope     \\
58895.29 & +41.09  & $i$    & 16.248               & 0.014  & Swope     \\
58895.29 & +41.09  & $i$    & 16.437               & 1.086  & LCO       \\
58895.43 & +41.23  & $i$    & 15.545               & 0.062  & Nickel    \\
58895.44 & +41.24  & $i$    & 19.07                & 1.086  & Nickel    \\
58896.29 & +42.09  & $i$    & 15.685               & 0.033  & Swope     \\
58897.31 & +43.11  & $i$    & 15.989               & 0.011  & Swope     \\
58898.24 & +44.04  & $i$    & 16.254               & 0.022  & Thacher   \\
58899.24 & +45.04  & $i$    & 16.477               & 0.035  & Thacher   \\
58900.35 & +46.15  & $i$    & 16.296               & 0.018  & Thacher   \\
58900.38 & +46.18  & $i$    & 18.472               & 1.086  & Nickel    \\
58902.24 & +48.04  & $i$    & 16.757               & 1.086  & LCO       \\
58902.26 & +48.06  & $i$    & 16.359               & 0.046  & Thacher   \\
58903.27 & +49.07  & $i$    & 16.487               & 0.018  & Swope     \\
58903.29 & +49.09  & $i$    & 16.334               & 0.03   & Thacher   \\
58904.32 & +50.12  & $i$    & 16.54                & 0.019  & Swope     \\
58904.35 & +50.15  & $i$    & 19.242               & 1.086  & Nickel    \\
58905.29 & +51.09  & $i$    & 16.65                & 0.015  & Swope     \\
58905.58 & +51.38  & $i$    & 16.491               & 0.154  & Thacher   \\
58906.1  & +51.9   & $i$    & 15.854               & 0.021  & LCO       \\
58906.1  & +51.9   & $i$    & 17.284               & 1.086  & LCO       \\
58906.28 & +52.08  & $i$    & 16.73                & 0.014  & Swope     \\
58907.36 & +53.16  & $i$    & 16.625               & 0.012  & Swope     \\
58908.3  & +54.1   & $i$    & 16.789               & 0.015  & Swope     \\
58908.3  & +54.1   & $i$    & 16.781               & 0.018  & Swope     \\
58909.36 & +55.16  & $i$    & 16.835               & 0.016  & Swope     \\
58911.2  & +57.0   & $i$    & 16.746               & 0.02   & Swope     \\
58912.27 & +58.07  & $i$    & 16.765               & 0.019  & Swope     \\
58919.14 & +64.94  & $i$    & 16.612               & 1.086  & LCO       \\
58923.14 & +68.94  & $i$    & 17.496               & 1.086  & LCO       \\
58923.27 & +69.07  & $i$    & 16.597               & 0.012  & Swope     \\
58929.5  & +75.3   & $i$    & 13.019               & 1.086  & LCO       \\
58929.5  & +75.3   & $i$    & 16.965               & 1.086  & LCO       \\
58935.64 & +81.44  & $i$    & 16.757               & 0.362  & LCO       \\
58935.64 & +81.44  & $i$    & 16.757               & 1.086  & LCO       \\
58943.46 & +89.26  & $i$    & 15.983               & 1.086  & LCO       \\
58943.46 & +89.26  & $i$    & 15.98                & 0.362  & LCO       \\
58952.44 & +98.24  & $i$    & 17.94                & 1.086  & LCO       \\
58954.18 & +99.98  & $i$    & 19.039               & 1.086  & Nickel    \\
58959.34 & +105.14 & $i$    & 17.754               & 1.086  & LCO       \\
58963.21 & +109.01 & $i$    & 18.522               & 1.086  & Nickel    \\
58966.35 & +112.15 & $i$    & 16.729               & 1.086  & LCO       \\
58974.11 & +119.91 & $i$    & 16.862               & 1.086  & LCO       \\
58980.76 & +126.56 & $i$    & 16.862               & 1.086  & LCO       \\
58988.32 & +134.12 & $i$    & 16.94                & 1.086  & LCO       \\
58996.5  & +142.3  & $i$    & 17.492               & 1.086  & LCO       \\
59002.75 & +148.55 & $i$    & 18.695               & 1.086  & LCO       \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering \caption {Optical and UV Photometry of SN~2020oi (Cont.)} \label{tbl:optical_phot2} 
\begin{tabular}{cccccc}
\hline
MJD      & Phase   & Band    & Magnitude                  & Uncertainty & Telescope \\ \hline \hline
59007.71 & +153.51 & $i$    & 18.651               & 1.086  & LCO       \\
59014.8  & +160.6  & $i$    & 18.729               & 1.086  & LCO       \\
59026.35 & +172.15 & $i$    & 17.578               & 1.086  & LCO       \\
59032.34 & +178.14 & $i$    & 20.198               & 1.086  & LCO       \\
59038.72 & +184.52 & $i$    & 19.823               & 1.086  & LCO       \\
59202.1  & +347.9  & $i$    & 18.455               & 1.086  & LCO       \\
59208.07 & +353.87 & $i$    & 17.918               & 1.086  & LCO       \\
59214.05 & +359.85 & $i$    & 18.207               & 1.086  & LCO       \\
59220.37 & +366.17 & $i$    & 18.003               & 1.086  & LCO       \\
59226.11 & +371.91 & $i$    & 17.11                & 1.086  & LCO       \\
59227.72 & +373.52 & $i$    & 18.462               & 1.086  & LCO       \\
59232.38 & +378.18 & $i$    & 16.679               & 1.086  & LCO       \\
59236.06 & +381.86 & $i$    & 17.263               & 1.086  & LCO       \\
59245.42 & +391.22 & $i$    & 18.522               & 1.086  & LCO       \\
59252.06 & +397.86 & $i$    & 17.571               & 1.086  & LCO       \\
59257.33 & +403.13 & $i$    & 19.021               & 1.086  & LCO       \\
59262.23 & +408.03 & $i$    & 18.372               & 1.086  & LCO       \\
59267.12 & +412.92 & $i$    & 16.947               & 1.086  & LCO       \\
58862.53 & +8.33   & $z$    & 14.266               & 0.027  & Thacher   \\
58864.34 & +10.14  & $z$    & 14.023               & 0.017  & Thacher   \\
58866.33 & +12.13  & $z$    & 13.975               & 0.033  & Thacher   \\
58867.36 & +13.16  & $z$    & 13.964               & 0.019  & Thacher   \\
58871.34 & +17.14  & $z$    & 14.191               & 0.02   & Thacher   \\
58872.34 & +18.14  & $z$    & 14.247               & 0.018  & Thacher   \\
58873.41 & +19.21  & $z$    & 14.294               & 0.016  & Thacher   \\
58874.29 & +20.09  & $z$    & 14.422               & 0.021  & Thacher   \\
58876.29 & +22.09  & $z$    & 14.538               & 0.038  & Thacher   \\
58878.29 & +24.09  & $z$    & 14.635               & 0.046  & Thacher   \\
58880.29 & +26.09  & $z$    & 14.951               & 0.023  & Thacher   \\
58881.29 & +27.09  & $z$    & 15.006               & 0.022  & Thacher   \\
58886.29 & +32.09  & $z$    & 15.227               & 0.032  & Thacher   \\
58890.29 & +36.09  & $z$    & 15.486               & 0.053  & Thacher   \\
58892.27 & +38.07  & $z$    & 15.414               & 0.034  & Thacher   \\
58893.25 & +39.05  & $z$    & 15.5                 & 0.039  & Thacher   \\
58894.26 & +40.06  & $z$    & 15.43                & 0.026  & Thacher   \\
58898.25 & +44.05  & $z$    & 15.519               & 0.032  & Thacher   \\
58899.24 & +45.04  & $z$    & 15.534               & 0.035  & Thacher   \\
58900.35 & +46.15  & $z$    & 15.508               & 0.03   & Thacher   \\
58903.3  & +49.1   & $z$    & 15.773               & 0.046  & Thacher   \\
58905.58 & +51.38  & $z$    & 15.592               & 0.149  & Thacher   \\
58942.52 & +88.32  & $z$    & 16.958               & 0.049  & PS1       \\ \hline
\end{tabular}
\end{table}
